ALCS: An Adaptive Latency Compensation Scheduler for Multipath TCP in Satellite-Terrestrial Integrated Networks

The Satellite-Terrestrial Integrated Network (STIN) enhances end-to-end transmission by simultaneously utilizing terrestrial and satellite networks, offering significant benefits in scenarios like emergency response and cross-continental communication. Low Earth Orbit (LEO) satellite networks offer reduced Round Trip Time (RTT) for long-distance data transmission and serve as a crucial backup during terrestrial network failures. Meanwhile, terrestrial networks are characterized by ample bandwidth resources and generally more stable link conditions. Therefore, integrating Multipath TCP (MPTCP) into STIN is vital for optimizing resource utilization and ensuring efficient data transfer by exploiting the complementary strengths of both networks. However, the inherent challenges of STIN, such as heterogeneity, instability, and handovers, pose difficulties for traditional multipath schedulers, which are typically designed for terrestrial networks. We propose a novel multipath data scheduling approach for STIN, Adaptive Latency Compensation Scheduler (ALCS), to address these issues. ALCS refines transmission latency estimates by incorporating RTT, congestion window size, inflight and queuing packets, and satellite trajectory information. It further employs adaptive mechanisms for latency compensation and proactive handover management. It further employs adaptive mechanisms for latency compensation and proactive handover management. Implemented in the MPTCP Linux Kernel and evaluated in a simulated STIN testbed, ALCS outperforms existing multipath schedulers, delivering faster data transmission and achieving throughput gains of 9.8% to 44.0% compared to benchmark algorithms.

==> body.tex <==
\section{Introduction}\label{intro}

% To be more precise, integrating both satellite and terrestrial links for data transmission within STIN offers substantial advantages. For example, in cases of terrestrial network outages caused by natural disasters or other unforeseen events, the satellite network can act as a vital backup, ensuring the continuity of data transmission. Furthermore, for long-distance communications, LEO satellites provide a distinct advantage by reducing Round Trip Time (RTT) compared to terrestrial links. As an illustration, the RTT between Chicago and Tokyo using Inter-Satellite Links (ISLs) is approximately 80 ms, which is 50 ms faster than the current Internet path and even 20 ms quicker than the optimal fiber route\cite{handley2019using}.

In recent years, the Satellite-Terrestrial Integrated Network (STIN) has emerged as a promising solution to meet the growing demand for seamless and ubiquitous connectivity\cite{yao2018space,8946626}. By leveraging the complementary strengths of satellite and terrestrial communication systems, STIN offers a robust and comprehensive approach to achieving global coverage while ensuring uninterrupted, high-quality communication. Low Earth Orbit (LEO) satellite networks, in particular, provide extensive global coverage, enabling connectivity in remote or underserved regions such as oceans, deserts, mountains, and polar regions---locations where terrestrial networks are not feasible \cite{8610423,8473481}. At the same time, terrestrial networks contribute higher bandwidth and more stable link conditions, particularly in densely populated areas where high-capacity, low-latency connections are crucial. This synergy enhances the overall performance and reliability of STIN.

The integration of both satellite and terrestrial links for data transmission within STIN delivers significant benefits. In cases of terrestrial network disruptions---whether caused by natural disasters or other unforeseen circumstances---satellite networks can serve as a critical fallback, ensuring the continuity of data transmission. Moreover, for long-distance communications, LEO satellites provide a distinct advantage by reducing Round Trip Time (RTT) compared to terrestrial networks. For example, the RTT between Chicago and Tokyo via Inter-Satellite Links (ISLs) is approximately 80 ms, which is 50 ms faster than the current Internet route and 20 ms quicker than the optimal fiber path \cite{handley2019using}.

The simultaneous utilization of satellite and terrestrial networks within STIN can be effectively managed through the deployment of the Multipath TCP (MPTCP) protocol \cite{rfc6182, rfc8684}. MPTCP enables concurrent data transmission over multiple network paths, significantly enhancing both throughput and transmission reliability. This approach has been widely adopted in various terrestrial networks, as demonstrated in \cite{dems, daps, blest, ecf, stms, sttf}. 
At the same time, MPTCP has also shown increasing potential in satellite communication environments \cite{SDN-enabled-LEO, du2015multipath}, optimizing resource usage and ensuring resilient data transmission across diverse network paths.
% While MPTCP has shown increasing promise in satellite communication environments \cite{SDN-enabled-LEO, du2015multipath}, optimizing resource usage and ensuring resilient data transmission across diverse network paths, research on MPTCP data scheduling specifically for satellite networks remains limited.

% Although research on MPTCP data scheduling for satellite networks is still scarce, MPTCP is being increasingly utilized in various satellite communication environments \cite{SDN-enabled-LEO, du2015multipath}, demonstrating its potential to optimize resource usage and ensure resilient data transmission across different network paths.

% The simultaneous use of both the satellite and terrestrial networks can be facilitated by deploying Multipath TCP (MPTCP) transmission protocol in the Satellite-Terrestrial Integrated Network (STIN).
% Multipath TCP (MPTCP) \cite{rfc6182, rfc8684} can exploit diverse paths concurrently to increase the network throughput and enhance transmission reliability, as already demonstrated in both terrestrial and satellite communication scenarios\cite{fleety-wifi-cellular, dems, SDN-enabled-LEO,du2015multipath}.

% Existing deployed MPTCP schedulers, such as the default minRTT scheduler\cite{mptcp-linux-kernel}, RoundRobin (RR) scheduler\cite{mptcp-linux-kernel}, Delay-Aware Packet Scheduler (DAPS)\cite{daps}, BLocking ESTimation-based scheduler (BLEST)\cite{blest}, Earliest Completion First (ECF) scheduler\cite{ecf}, and so on, are limited to terrestrial networks using cellular and Wi-Fi paths. 
% The minRTT scheduler prioritizes the subflow with the minimum observed RTT, while the RR scheduler distributes traffic fairly without considering network conditions. In contrast, the DAPS scheduler dynamically assigns packets based on forward delay and Congestion Window size (CWND) to optimize performance. Furthermore, the BLEST scheduler estimates blocking time to select the highest throughput path, and the ECF scheduler prioritizes the fastest predicted completion time by looking beyond just RTT or blocking.

% LEO satellite networks can provide lower Round Trip Time (RTT) when it comes to long-distance communication. For instance, the Chicago-Tokyo RTT using Inter-Satellite Links (ISLs) is around 80 ms, which beats the current Internet path by 50 ms and is even 20 ms faster than the optimal fiber path\cite{handley2019using}. 
% Also, simply utilizing limited resources in terrestrial communication networks makes it difficult to support the massive Quality of Service (QoS) aware requirements and it is hard to guarantee seamless coverage in far remote regions\cite{wang2019convergence}.
% However, the rapid movement and frequent handover of LEO satellites can lead to constant changes in network topology, resulting in service interruptions and performance deterioration. Leveraging terrestrial and LEO satellite networks simultaneously could improve the robustness of connection through seamless transitions between satellite and terrestrial paths. To this end, a multipath transmission scheme is imperative.

% Multipath TCP (MPTCP)\cite{rfc6182, rfc8684} can exploit diverse paths concurrently to increase the network throughput and enhance transmission reliability, as already demonstrated in both terrestrial and satellite communication scenarios\cite{fleety-wifi-cellular, dems, SDN-enabled-LEO,du2015multipath}. 

% However, the dynamic movement and rapidly changing link conditions of LEO satellites can lead to frequent shifts in network topology, potentially causing service disruptions. This underscores the necessity of integrating satellite and terrestrial networks within STIN to maintain stable connectivity and consistent performance across various environments.

However, research on MPTCP data scheduling specifically for satellite networks remains limited. The deployment of MPTCP within STIN introduces several challenges due to the network's inherent complexities. These include significant differences in path characteristics such as latency, bandwidth, and packet loss rates, high temporal variability in network conditions, and the constant mobility of LEO satellites. These factors make it difficult to maintain stable and efficient data transmission, posing three primary challenges for MPTCP implementation within STIN:
% However, due to the inherent complexities of STIN, including substantial differences in path characteristics, high temporal variability, and the constant mobility of LEO satellites, deploying the MPTCP protocol within STIN for efficient data transmission presents three key challenges:
\begin{itemize}
	\item \textbf{Severe heterogeneity}. The path characteristics can vary significantly between satellite and terrestrial paths in the STIN environment. In addition to significant RTT discrepancies, satellite links often have lower bandwidth compared to terrestrial paths \cite{1677596}. This pronounced path heterogeneity can lead to out-of-order packet delivery and receiver buffer blocking, degrading overall throughput and transmission efficiency.
	\item \textbf{High volatility}. LEO satellite networks, such as Starlink, are highly dynamic, with significant temporal variability in path characteristics. Taking Starlink as an example, the latency variation reaches around 3.8 times that of terrestrial networks while the throughput standard deviation achieves 50.71\% \cite{2023-starlink-measurement}. Moreover, Ground-to-Satellite Links (GSL) are sensitive to weather conditions and signal interference,  further complicating network stability and predictability.
    \item \textbf{Frequent Handover}. Due to the constant movement of LEO satellites, frequent handovers are inherent in satellite networks \cite{mptcp-handover}. These handovers can result in packet drops and increased retransmissions, negatively impacting transmission efficiency and overall performance.
\end{itemize} 

% In contrast, the BLEST scheduler estimates the blocking time for each subflow based on observed performance metrics, aiming to select the subflow likely to provide the highest throughput, rather than just the lowest latency. Furthermore, the ECF scheduler prioritizes the subflow predicted to complete the data transfer the fastest, considering factors beyond just RTT or blocking time. 
% The choice of the most suitable scheduler ultimately depends on the specific network environment and requirements, necessitating evaluation and adaptation to ensure optimal MPTCP performance.
% When sending data, the minRTT scheduler will preferentially select the subflow with the currently observed minimum RTT to transmit the data. This can lead to a situation where the overall throughput of the MPTCP connection is limited by the capacity of the lowest-RTT subflow, even if other subflows have higher available bandwidth. As an alternative to the default minRTT scheduler, the round-robin scheduler selects the available subflows in a circular, sequential manner for data transmission, ensuring fair distribution of traffic across the available subflows. However, without considering the current network conditions, the round-robin scheduler may not always select the most optimal subflow for a given data transmission.
% The BLEST scheduler estimates the blocking time for each subflow based on observed network performance metrics, aiming to select the subflow that is likely to provide the highest throughput, rather than just the lowest latency.
% Moreover, ECF prioritizes the subflow that is predicted to complete the data transfer the fastest, rather than just focusing on the lowest RTT or blocking time.

The distinctive characteristics of STIN present significant challenges for traditional MPTCP scheduling algorithms.
Due to the limited research on MPTCP data scheduling specifically for satellite networks, the schedulers listed here are primarily designed for terrestrial networks---where paths typically consist of cellular or Wi-Fi connections---including the default minRTT scheduler\cite{mptcp-linux-kernel}, RoundRobin (RR) scheduler\cite{mptcp-linux-kernel}, Delay-Aware Packet Scheduler (DAPS)\cite{daps}, BLocking ESTimation-based scheduler (BLEST)\cite{blest}, and Earliest Completion First (ECF) scheduler\cite{ecf}. 
% As research on MPTCP data scheduling specifically for satellite networks remains limited, these schedulers are primarily designed for terrestrial networks, where paths typically consist of cellular or Wi-Fi connections, and may struggle to handle STIN's complexities. 
The minRTT scheduler prioritizes subflows with the lowest RTT, often underestimating the inherent delays of satellite links. Similarly, the RR scheduler distributes traffic equally across paths, failing to consider the substantial differences in subflow capacities. BLEST, which adjusts traffic based on observed network conditions, may struggle to react swiftly to the rapid fluctuations in STIN. Even the more sophisticated ECF scheduler, which considers factors beyond RTT to estimate completion times, can falter under STIN’s frequent handovers and dynamic satellite link conditions. These limitations highlight the need for specialized scheduling strategies that address the unique challenges of STIN to optimize MPTCP performance in such integrated and complex network environments.

%However, since the STIN is much more heterogeneous and dynamic than the terrestrial networks, these past approaches cannot be directly transplanted into STIN.

%In this paper, we introduce a new MPTCP scheduler tailored for STIN to maximize network resource utilization while ensuring data transmission continuity, which is called XXX. To realize the objective, XXX monitors multiple characteristics of established subflows (satellite paths and terrestrial paths), including RTT estimates, congestion windows ($CWNDs$), the amount of queuing packets, and also maintains the LEO satellite handover timetable as the moving trajectories are predictable. Combing these metrics, XXX estimates each subflow's quality and dynamically adjusts the amount of data packets that need scheduling to mitigate the packet out-of-order in the receive buffer due to path heterogeneity. Additionally, since the satellite trajectory is predictable, XXX would disable the satellite path that is to be broken due to the oncoming handover in advance, thus preventing unnecessary packet loss. In specific, XXX is designed with the following properties:
%\begin{itemize}
%    \item To estimate the qualities of the satellite path and terrestrial path in a reasonable manner, XXX continuously monitors their RTT and CWND that embodies the available bandwidth and periodically calculates the packet loss rate. Based on these metrics and the amount of data queued in the send buffer, XXX determines if it is necessary to split the queued packets into two segments and then decides the amount of data that needs to be scheduled into satellite path and terrestrial path respectively.
    % LEO satellites move in predictable orbits.
%    \item Given frequent handovers of LEO satellites, XXX maintains the trajectory information of LEO satellites and proactively disables the satellite path in advance when a handover is anticipated. In other words, only the terrestrial path would be utilized under this circumstance, which means that multipath transmission degrades into single-path transmission.
%    \item Due to the susceptibility of the GSL to disconnection, XXX incorporates a rapid loss or fault detection and recovery mechanism. Once short-duration consecutive packet losses are detected on the satellite link, the path will be disabled either. All the lost packets will be reinjected in the terrestrial path promptly in order to alleviate the blocking of receiver buffer.
%\end{itemize}

In this paper, we propose an Adaptive Latency Compensation Scheduler (ALCS), a novel multipath packet scheduler specifically designed for STIN. ALCS aims to minimize data transmission time, increase the overall network throughput, and enhance transmission reliability across satellite and terrestrial network paths. 
The core innovation of ALCS lies in its ability to adaptively compensate for estimated packet transmission delays in STIN while proactively deactivating the satellite path prior to handovers. This approach takes into account RTT fluctuations and satellite movement, delivering more reliable and efficient data transfer. By optimizing the use of satellite network resources alongside terrestrial networks, ALCS allows for smoother transitions and enhanced performance in dynamic STIN environments.
% The core innovation of ALCS lies in its ability to adaptively compensate for estimated packet transmission delays in STIN and proactively deactivate the satellite path before handover, accounting for RTT fluctuations and satellite movement. This allows for optimal use of satellite bandwidth alongside terrestrial networks, ensuring more reliable and efficient data transfer.
% to estimate the tranission delay of data packets more precisely in STIN considering the RTT fluctuation and satellite movement and to increase the utilization of both satellite network bandwidth resources and terrestrial networks. 

The main contributions of this paper are summarized as follows:
\begin{itemize}
    \item We introduce an MPTCP data transmission framework tailored for STIN and analyze the performance degradation of traditional MPTCP schedulers when deployed in this environment.    
    \item We design a novel multipath scheduler, ALCS, that addresses path heterogeneity, RTT fluctuations, and handovers caused by satellite movement. By evaluating the transmission delays, ALCS selects the most appropriate path for the current data segments, ensuring reliable and efficient delivery in rapidly changing network conditions.
    \item We implement the ALCS scheduler in the Linux Kernel. Additionally, we build a flexible and scalable testbed using Docker containers and Python scripts, enabling a thorough study of different scheduler behaviors under diverse STIN conditions.
    % An implementation of our proposed scheduler is realized in the Linux Kernel. Moreover, by leveraging Docker containers and Python script, we establish a flexible and scalable testbed that enables us to study the behavior and performance of different schedulers in the simulated STIN under various conditions and configurations. 
    \item We evaluate the performance of ALCS against several MPTCP schedulers, including minRTT, RR, BLEST, and ECF, in a custom-built experimental testbed. The results demonstrate that our proposed ALCS improves overall performance ranging from 9.8\% to 44.0\% across various metrics.
\end{itemize}

The remainder of this paper is structured as follows. Section \ref{bg} provides the necessary background on the MPTCP protocol in the context of STIN, highlights the unique characteristics of STIN, and examines the performance limitations of traditional schedulers in the STIN environment. In Section \ref{design}, we present the design of our proposed ALCS scheduler. Implementation details and the experimental testbed setup are provided in Section \ref{testbed}, followed by evaluations of ALCS and other scheduling algorithms in Section \ref{results}. Discussions, limitations, and future work are given in Section \ref{discussion}. The relevant related work is reviewed in Section \ref{related-work}, and conclusions are drawn in Section \ref{conclusion}.

% \section{Background and Motivation}\label{bg}
% In this section, a brief introduction to the MPTCP protocol for data transmission in STIN is provided in the first place, followed by a concise review of several traditional MPTCP schedulers.

% \subsection{multipath TCP Protocol for STIN}

\section{Implementation and Challenges of MPTCP in STIN} \label{bg}
% In this section, we first present the MPTCP communication diagram for STIN. Subsequently, we provide a brief introduction of inherent characteristics of STIN, which sets the stage for an examination of the performance degradation exhibited by various conventional MPTCP scheduling algorithms.


In this section, we first present the MPTCP communication diagram for STIN, followed by an overview of one main inherent characteristic of STIN that challenges the effectiveness of MPTCP. Lastly, we analyze the performance degradation seen in various conventional MPTCP scheduling algorithms.


\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{mptcp-structure.pdf}
    \caption{MPTCP data transmission diagram for STIN.}
    \label{mptcp-structure}
\end{figure}

\subsection{MPTCP for STIN}
% The MPTCP protocol functions between the transport and application layers, enabling the simultaneous use of various network paths for data transfer. It seamlessly integrates these paths, yet presents itself as a single TCP protocol at higher levels. 
% At the transport layer, MPTCP is bifurcated into two layers. The upper layer is responsible for network path management, while the lower layer divides packets into multiple subflows for transmission over various available paths. Each sub-flow behaves as if it were a single TCP flow. The communication mechanism of MPTCP primarily encompasses connection initialization, establishment of available subflows, data transmission, and connection termination. 

% The MPTCP protocol operates between the transport and application layers, dividing packets into multiple subflows for transmission across various available paths. Each sub-flow behaves as if it were a single TCP flow. The communication mechanism of MPTCP primarily encompasses connection initialization, establishment of available subflows, data transmission, and connection termination. 

The MPTCP protocol operates between the transport and application layers, splitting packets into multiple subflows for transmission across different available paths. Each subflow functions independently, resembling a standalone TCP flow. The MPTCP communication process primarily involves connection initialization, the establishment of available subflows, data transmission, and connection termination.

Fig.~\ref{mptcp-structure} illustrates the MPTCP architecture within a STIN, leveraging both satellite and terrestrial networks concurrently. The key communication steps within this STIN context are detailed as follows:

\begin{itemize}
    \item[1] MPTCP first establishes an initial TCP connection, similar to the traditional single TCP connection setup process, which includes the standard three-way handshake. This step is essential for configuring communication parameters and capabilities between the source and destination.
    \item[2] Upon completing the initial connection, MPTCP identifies all available sub-paths, which can be established across different network interfaces, physical routes, and devices. In the case of multiple end-to-end paths, such as terrestrial and satellite links in STIN, corresponding subflows are created. These subflows are used for parallel data transmission, improving reliability and efficiency.
    \item[3] 
    % Afterward, MPTCP simultaneously transmits the data through different subflows. A data scheduler determines the best subflow on which to transmit packets. Therefore, it is non-trivial to design a feasible and reasonable scheduler for effective data transmission in STIN.
    Following the establishment of subflows, MPTCP transmits data concurrently across the different paths. A data scheduler is responsible for selecting the optimal subflow for packet transmission. Consequently, designing an efficient and robust scheduler is critical for ensuring effective data transmission within STIN.
    \item[4] After data transmission is completed, MPTCP terminates the connection, following a procedure similar to the traditional TCP termination process.
\end{itemize}

% In this paper, we focus on the design of a STIN-tailored MPTCP data scheduler, as highlighted in step 3.
% In general, the MPTCP study can be divided into three main sections, including path manager, data scheduler, and congestion controller. 

As emphasized in step 3, efficient multipath data scheduling is critical to improving the performance and effectiveness of MPTCP in real-world networks. By intelligently distributing data traffic based on path characteristics, congestion levels, and application requirements, multipath scheduling algorithms can optimize resource utilization and significantly enhance the end-user experience. However, several inherent attributes of STIN pose significant challenges to traditional data scheduling methods primarily designed for terrestrial networks.

% \textbf{minRTT}\cite{mptcp-linux-kernel}: As the default MPTCP scheduler, minRTT, as its name suggests, favors the subflow with the currently observed minimum RTT for data transmission. However, this approach can limit the overall throughput to the capacity of the lowest-RTT subflow, even if other available paths have higher bandwidths that could be better leveraged.

% \textbf{RR}\cite{mptcp-linux-kernel}: To ensure equitable data distribution, the RR scheduler evenly divides traffic among all active subflows, disregarding the actual network conditions. Consequently, it may fail to consistently choose the most efficient subflow for transmission, potentially leading to inefficient usage of the network resources.

% \textbf{BLEST}\cite{blest}: The BLEST scheduler, on the other hand, takes a more sophisticated approach. It estimates the blocking time for each subflow based on observed network performance metrics. By extending its scope beyond round-trip time to include other relevant factors, the method is designed to identify the subflow with the potential for the greatest overall throughput, rather than merely prioritizing the path with the lowest current latency.

% \textbf{ECF}\cite{ecf}: Moreover, the ECF scheduler strategically prioritizes subflows that are anticipated to complete data transfers most swiftly, taking into account a broader range of factors than just RTT or blocking time. By dynamically estimating the completion time for each available subflow, this advanced scheduling technique aims to maximize the overall throughput, overcoming the limitations of techniques focused solely on latency-based metrics. 

% These existing multipath scheduling approaches are predominantly designed for wireless network environments, primarily considering the characteristics of Wi-Fi and cellular network paths. As a result, their direct application within the STIN environment might not be suitable, given the distinct requirements and dynamic network conditions of STIN. More details and analyses are given in Section \ref{motivation}.

% \section{Motivation}\label{motivation}
% In this section, we first introduce the key features of the STIN architecture and examine its impacts on network performance. We then present a brief analysis of the performance degradation observed with traditional MPTCP scheduling approaches when deployed in this particular STIN environment.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{rtt-ping.png}
    \caption{Latency dynamics in a simulated STIN environment.}
    \label{fig:sat-rtt}
\end{figure}

\subsection{Characteristics of STIN}
% As mentioned in Section \ref{intro}, one well-known challenge in STIN is the handover issue raised by the movement of satellites\cite{mpquic}. As the network topology rapidly changes, the frequent handovers between satellites and between satellites and ground stations can dramatically alter the network conditions. To be specific, satellite paths can appear and disappear from time to time, while their latency, bandwidth, and reliability characteristics may fluctuate rapidly.

% At the same time, the inherent variability of satellite link RTT poses additional challenges. While LEO constellations can provide lower long-distance end-to-end latency compared to terrestrial systems, the RTT of individual satellite links is highly susceptible to a variety of external factors beyond just satellite movement, such as atmospheric conditions, interference, satellite loading, hardware issues, and ground station conditions. 
% This high degree of RTT variability adds further complexity.
% Furthermore, the inherent variability of satellite link RTT poses additional challenges. While LEO constellations can provide lower absolute RTT compared to legacy satellite systems, the RTT of individual satellite links can still exhibit significant fluctuations due to factors like changing distance to the satellite, atmospheric conditions, and network congestion. These RTT variations can disrupt the timing-sensitive operations of traditional multipath schedulers, leading to suboptimal packet sequencing, increased jitter, and reduced overall performance.

As discussed in Section \ref{intro}, a major challenge in STIN is the handover issue caused by satellite movement. Frequent handovers between satellites and ground stations, or across satellites, can have a substantial impact on link conditions. For example, in cases where a communication session depends on a single end-to-end satellite path, a handover may result in disconnection, disrupting the continuity of transmission. Conversely, in systems with multiple satellite paths, ISL handovers can introduce fluctuations in RTT and bandwidth variability, which may degrade the overall quality of service.

% To summarize, handover challenges in STIN systems can either lead to satellite communication disruptions in single-path satellite network scenarios or result in performance variability due to RTT and bandwidth fluctuations in multipath satellite networks.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.65\columnwidth]{rtt-cdf.png}
    \caption{CDF of the difference between the maximum and minimum RTTs of the satellite path.}
    \label{fig:sat-rtt-cdf}
\end{figure}

% Fig. \ref{fig:sat-rtt} demonstrates the significant fluctuations in RTT experienced in an end-to-end connection utilizing ISLs in our custom-built testbed (see details in Section \ref{testbed}). 
% Fig. \ref{fig:sat-rtt} demonstrates the RTT fluctuations of satellite connection in our custom-built testbed (see details in Section \ref{testbed}). To efficiently showcase the RTT characteristics of the satellite link within a constrained test duration, we expedite the pace of satellite movement in the examined testbed. This enables a 300-second ping involving long-distance communication, providing insights into RTT performance under accelerated conditions that mimic real LEO satellite dynamics.

Fig. \ref{fig:sat-rtt} presents the RTT fluctuations of a satellite connection observed in our custom-built testbed (see Section \ref{testbed} for details). To effectively capture the RTT characteristics within a limited test period, we accelerate the satellite movement in the testbed. This approach enables a 300-second ping test over long-distance communication, offering insights into RTT performance under conditions that simulate real LEO satellite dynamics at an accelerated rate. As shown in Fig. \ref{fig:sat-rtt}, the predominantly stable and low RTT, averaging around 60 ms, highlights the satellite network's potential for reduced latency in long-distance communications, in contrast to terrestrial networks, which typically exhibit RTT values exceeding 100 ms.

% we observe some stable and low RTT periods predominantly around 60 ms, which underscores the satellite network's potential for lower latency in long-distance communications over terrestrial networks, with the latter exhibiting RTT values consistently above 100 ms. 

Nevertheless, the RTT of the satellite path exhibits significant fluctuations, including notable spikes labeled as ``disconnection" events. These spikes are primarily attributed to handovers between LEO satellites, particularly when a single satellite path is in use. Such handovers can cause temporary disconnections and RTT values spiking well above the baseline. This recurring pattern of handover-induced spikes undermines the overall quality and reliability of the connection, leading to unpredictable service interruptions and degraded performance. Additionally, there are instances where RTT shifts from approximately 60 ms to 40 ms, which are associated with ISL handovers when multiple satellite paths are active in the test environment.

To illustrate the variability in RTT experienced by the satellite link, we present the Cumulative Distribution Function (CDF) of the difference between the maximum and minimum RTTs observed on the satellite path during the 300-second ping test, as shown in  Fig. \ref{fig:sat-rtt-cdf}. The CDF indicates that RTT variations exceeding 10 ms occur with a probability of approximately 0.4, highlighting the significant likelihood of such fluctuations. Furthermore, there is a small but notable chance of encountering RTT variations exceeding 20 ms, emphasizing the inherent volatility of satellite communication links.

Therefore, addressing the varying RTT challenges through advanced mobility management and multipath transmission schemes is essential to fully leverage the benefits of STIN architectures. Effective solutions can ensure seamless, high-quality connectivity despite the dynamic and constantly evolving network topology.
% The RTT exhibits significant fluctuations, with several distinct spikes marked as "handover" events. These handover periods, caused by the constant movement of LEO satellites, lead to severe disruptions in the network connection, with RTT values spiking well above the baseline.
% However, it also displays periods of relatively stable and low RTT, suggesting the potential benefits of the satellite network component, such as its low-latency capabilities when involving long-distance communication. Yet, the consistent pattern of handover-induced spikes undermines the overall quality and reliability of the connection, as users experience unpredictable service interruptions and degraded performance. Addressing these handover challenges through advanced mobility management and multipath transmission schemes will be crucial to fully realize the advantages of integrated satellite-terrestrial architectures and provide seamless, high-quality connectivity, even in the face of a dynamic and constantly evolving network topology.

\subsection{Performance Degradation}

Most existing multipath schedulers rely on assumptions of relatively stable path characteristics and availability. However, frequent satellite handovers in STIN scenarios can drastically alter network conditions, making these assumptions invalid. As a result, traditional scheduling algorithms, which optimize based on time-invariant path metrics, may perform poorly, leading to suboptimal resource utilization and potential service disruptions during communications.

\subsubsection{\textbf{Severe Retransmission due to Handover-induced Disconnection}} We conduct a comprehensive evaluation of various MPTCP schedulers in our custom-built testbed, focusing on a single satellite path scenario. When data packets are transmitted over a satellite path nearing handover, the likelihood of packet loss increases dramatically due to the imminent disconnection. This packet loss triggers a cascade of retransmissions, consuming additional bandwidth and system resources, while also introducing latency. The cumulative effect of these retransmissions can significantly degrade the overall transmission performance, leading to slower data delivery rates and higher error rates.

\begin{table}[t!]
    \centering
    \caption{Packet Retransmission due to LEO Satellite Handovers.}
    % \resizebox{\columnwidth}{12mm}{
    \begin{tabular}{m{2.5cm}<{\centering}|m{5.3cm}<{\centering}}
        \hline
        \textbf{MPTCP scheduler} & \textbf{retransmission packets caused by handover / total retransmissions} \\
        \hline
        minRTT & 215 / 230 (93.48\%) \\
        RR               & 400 / 437 (91.53\%) \\
        BLEST            & 810 / 822 (98.54\%) \\
        ECF              & 286 / 296 (96.62\%) \\
        \hline 
    \end{tabular}
    \label{tab:retrans}
\end{table}

As illustrated in Table \ref{tab:retrans}, traditional MPTCP schedulers, including minRTT, RR, BLEST, and ECF, suffer from substantial performance degradation due to packet loss and retransmission triggered by satellite handovers. Notably, a vast majority—between 91\% and 98\%—of all retransmissions stem from these handovers, highlighting the inability of existing MPTCP scheduling strategies to effectively mitigate data loss during satellite link transitions. 

In scenarios where data segments are allocated to a satellite path nearing handover, most of these packets may require retransmission as they are lost during the temporary disconnection of the satellite link. While retransmission over the terrestrial path can help ensure seamless transmission at the application layer, this approach comes at the cost of consuming additional terrestrial bandwidth resources. On the other hand, retransmitting via the satellite path forces the receiver to wait until the link is restored, which can lead to significant delays and out-of-order delivery.
This trade-off underscores the importance of proactively preventing packet loss due to handovers, rather than relying on reactive retransmission strategies.

% As clearly demonstrated in Table \ref{tab:performance-degradation}, the conventional MPTCP schedulers experience significant performance degradation when confronted with packet loss and retransmission issues induced by satellite handover. Across the different schedulers - the default (minRTT), RR, BLEST, and ECF - a significant majority, ranging from 93\% to 98\%, of the total retransmissions are caused by the handover process. This indicates that the existing MPTCP scheduling strategies are unable to effectively manage the data losses occurring during satellite handovers.

\subsubsection{\textbf{Performance Degradation Still Occurs in Non-Disconnection Scenarios}}

To evaluate the impact of STIN's inherent heterogeneity and satellite link dynamics, we also analyze the performance of various MPTCP schedulers in scenarios where satellite link disconnections are absent throughout the data transmission process.

Table \ref{tab:performance-degradation} presents a comparative analysis of four MPTCP schedulers under these conditions.
We assess the transmission completion time and average throughput while transferring a 100MB file using these schedulers, ensuring no handover events occur during the process. It is observed that the default minRTT scheduler has the longest transfer duration and the lowest overall throughput among the four schedulers. Meanwhile, the RR, BLEST, and ECF schedulers exhibit similar performance, with transmission completion times of approximately 48 seconds and average throughputs of around 2.319MB/s. This suggests that ECF and BLEST may not maintain their advantage in the highly dynamic and heterogeneous STIN environment. The reliance of ECF and BLEST on RTT estimates, which are prone to significant fluctuation in satellite paths, likely impacts the accuracy of their estimations and, consequently, their effectiveness.

Thus, it is crucial to develop multipath data schedulers specifically designed to address the unique challenges of STIN environments.

\begin{table}[t!]
    \centering
    \caption{Performance Comparison in Non-handover STIN Scenarios.}
    % \resizebox{\columnwidth}{12mm}{
    \begin{tabular}{m{2.5cm}<{\centering}|m{2.1cm}<{\centering}|m{3.1cm}<{\centering}}
        \hline
        \textbf{MPTCP scheduler} & \textbf{completion time (s)} & \textbf{average throughput (MB/s)} \\
        \hline
        minRTT & 56.779 & \num{1.988} \\
        RR               & 48.462 & \num{2.319} \\
        BLEST            & 48.453 & \num{2.319} \\
        ECF              & 48.018 & \num{2.319} \\
        \hline 
    \end{tabular}
    \label{tab:performance-degradation}
\end{table}

\section{Algorithm Design}\label{design}

This section details the design of our proposed scheduling algorithm, ALCS. We begin with an overview of ALCS, outlining its foundational principles and objectives. Following this, we examine the three pivotal components that form the core of the ALCS framework.

% This section presents the details of our proposed scheduling algorithm, ALCS. ALCS leverages the advantages from prior scheduling approaches and refines them by integrating considerations for the unique features of the STIN environment. The goal of ALCS is to harness the complementary capabilities of satellite and terrestrial links to deliver enhanced end-to-end communication reliability and efficiency for users.
%The proposed scheduler inherits the benefits of some existing schedulers while addressing the drawbacks by considering the specific features of the STIN environment.

\subsection{Design Overview}

To elaborate, we first define the following variables. The variable $S_f$ denotes the fastest subflow, while $S_s$ represents the slower subflow among the available paths. $rtt_f$ and $cwnd_f$ refer to the RTT and CWND of $S_f$, whereas $rtt_s$ and $cwnd_s$ are for $S_s$. $\Delta_f$ and $\Delta_s$ denote the variations of $rtt_f$ and $rtt_s$, respectively. Furthermore, $tl_f$ and $tl_s$ denote the estimated transmission latencies for $S_f$ and $S_s$, including any waiting time and the transmission delay for data segments scheduled over these subflows. $\sigma_f$ and $\sigma_s$ are latency compensation factors used to refine the estimated latencies. The variable $T_u$ denotes the update interval for revising the compensation factors $\sigma_f$ and $\sigma_s$. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth]{ALCS-flowchart-v2.png}
    \caption{Flowchart diagram of the proposed ALCS.}
    \label{fig:ALCS-flowchart}
\end{figure}

% To illustrate, Fig. \ref{fig:ALCS-flowchart} indicates the high-level design overview of our proposed ALCS, containing three main sections including latency estimation for two subflows, adaptive estimated latency compensation, and proactive handover management.

% The ALCS algorithm aims to leverage the complementary strengths of satellite and terrestrial links to enhance end-to-end communication reliability and efficiency. Fig. \ref{fig:ALCS-flowchart} indicates the high-level design overview of our proposed ALCS, containing three main sections including latency estimation for satellite and terrestrial paths, adaptive latency compensation, and proactive handover management. 
% ALCS calculates the waiting and transmission latencies $tl_f$ and $tl_s$ over both $S_f$ and $S_s$ in the first place, taking into account path metrics such as RTT, CWND, and other characteristic metrics. Based on these calculations, ALCS strategically assigns packets to the subflow predicted to deliver packets to the receiver more swiftly, a strategy that bears a resemblance to the ECF and STFT schedulers. To enhance this process, ALCS incorporates a latency estimation compensation mechanism. This mechanism introduces a latency compensation factor, $\sigma$, which is designed to refine the latency estimation and address potential inaccuracies that may arise from the volatility of satellite links. Furthermore, a proactive handover management mechanism is also integrated into ALCS to mitigate the negative impacts of satellite handovers.

The general workflow of the ALCS scheduling algorithm is outlined in Fig. \ref{fig:ALCS-flowchart} and can be summarized as follows: 1) Identify all available subflows, including both satellite and terrestrial paths within the STIN environment, designating the faster path as $S_f$ and the slower one as $S_s$; 2) Return $S_f$ if it has available CWND capacity; 3) Otherwise estimate the transmission latencies $tl_f$ and $tl_s$ for both $S_f$ and $S_s$, using path metrics $rtt_f, cwnd_f, rtt_s, cwnd_s$, along with inflight packet counts and queuing lengths; 4) Refine the estimated latencies by incorporating latency compensation factors $\sigma_f$ and $\sigma_s$, which are updated at each update interval $T_u$; 5) Based on these calculations, determine whether to proceed with $S_f$ immediately or defer transmission until $S_f$ becomes available again.
It is important to note that in the long-distance communication scenarios under study, the satellite path utilizing ISLs typically exhibits a lower RTT than the terrestrial path. Consequently, $S_f$ predominantly signifies the satellite path in this context.

% we denote the faster subflow and the slower subflow as $S_f$ and $S_s$, respectively. Accordingly, $rtt_f$ and $rtt_s$ represent the RTTs of subflows $S_f$ and $S_s$, while $cwnd_f$ and $cwnd_s$ denote their CWNDs. It is noteworthy that in the long-distance communication scenarios we are examining, the satellite path utilizing ISLs typically exhibits a lower RTT compared to the terrestrial path. Consequently, $S_f$ predominantly signifies the satellite path in this context.

% Fig. \ref{fig:ALCS-flowchart} indicates the overview design of our proposed ALCS, containing these three main sections including latency estimation for two subflows, adaptive estimated latency compensation, and proactive handover management. The general workflow of the ALCS scheduling algorithm can be summarized as follows: 1) Identify all available subflows, including both satellite and terrestrial paths in the STIN scenario, and designate the faster path as $S_f$ and the slower as $S_s$; 2) Return $S_f$ if it has available $cwnd$; 3) Otherwise estimate transmission latencies $tl_f$ and $tl_s$ for both $S_f$ and $S_s$ based on path characteristic metrics; 4) Return the subflow that is expected to result in a shorter transfer delay. The latency compensation factors, $\sigma_f$ and $\sigma_s$, are adaptively adjusted at each update interval $T_u$.
% The general steps of ALCS scheduling algorithm can be concluded as: 1) find all available subflows including satellite path and terrestrial path in STIN scenario and mark the faster path $S_f$ and the slower one $S_s$; 2) return $S_f$ if $S_f$ having available $cwnd$; 3) estimate transmission latencies for both $S_f$ and $S_s$ using Eq \ref{eq:estimate-tlf} and \ref{eq:estimate-tls}; 4) return the subflow that is expected to achieve shorter transfer delay. The latency compensation factors $\sigma_f$ and $\sigma_s$ are updated at each update interval $T_u$.
% Specifically, the satellite path, typically identified as the faster subflow $S_f$, is scheduled for deactivation in anticipation of an imminent handover.
% ALCS leverages the advantages from prior scheduling approaches and refines them by integrating considerations for the unique features of the STIN environment.
% The goal of ALCS is to harness the complementary capabilities of satellite and terrestrial links to deliver enhanced end-to-end communication reliability and efficiency for users.

% We assume that $k$ packet segments in the MPTCP connection level send buffer are waiting to be scheduled to the best available subflow. Similar to the default minRTT scheduler, if the fastest subflow\textemdash characterized by the minimal RTT\textemdash has available CWND space, ALCS would readily assign the packets to that subflow. However, in cases where the faster subflow $S_f$ lacks sufficient CWND space, our proposed approach would not allocate the data packets in the send buffer to the slower subflow $S_s$ immediately.

% Instead, ALCS calculates the waiting and transmission latencies $tl_f$ and $tl_s$ over both $S_f$ and $S_s$ in the first place, taking into account path metrics such as RTT, CWND, and other characteristic metrics. Based on these calculations, ALCS strategically assigns packets to the subflow predicted to deliver packets to the receiver more swiftly, a strategy that bears a resemblance to the ECF and STFT schedulers. To enhance this process, ALCS incorporates a latency estimation compensation mechanism. This mechanism introduces a latency compensation factor, $\sigma$, which is designed to refine the latency estimation and address potential inaccuracies that may arise from the volatility of satellite links. Furthermore, a proactive handover management mechanism is also integrated into ALCS to mitigate the negative impacts of satellite handovers.

The ALCS algorithm is designed to capitalize on the complementary strengths of satellite and terrestrial networks, aiming to enhance the reliability and efficiency of end-to-end communications. To this end, ALCS builds on the strengths of existing scheduling methods while introducing enhancements tailored to the specific challenges of the STIN environment. These challenges, as outlined in Section \ref{intro}, include significant network heterogeneity, high volatility in link quality, and frequent handovers. As depicted in Figure \ref{fig:ALCS-flowchart}, ALCS is structured around three key components: latency estimation for satellite and terrestrial paths, adaptive estimated latency compensation to fine-tune performance, and proactive handover management to ensure uninterrupted connectivity.
The strategies employed by each of these three components to address the corresponding challenges are listed below.
\begin{itemize}
    \item \textbf{Latency Estimation for Satellite and Terrestrial Paths}: Given the inherent differences between LEO satellite networks and terrestrial networks, ALCS implements a mechanism to estimate the transmission latency of data segments across both paths. This estimation factors in various network dynamics, such as RTT, CWND, inflight packets, and queue lengths, enabling the scheduler to make informed decisions based on real-time path conditions.   
    \item \textbf{Adaptive Estimated Latency Compensation}: To address performance issues arising from fluctuating satellite links, ALCS introduces an adaptive latency compensation mechanism. This component updates the latency compensation factors by periodically comparing the actual and estimated latencies. In this manner, it refines the latency estimation, thereby mitigating the adverse effects caused by the variability of link conditions.    
    \item \textbf{Proactive Handover Management}: Leveraging the predictable movement patterns of LEO satellites, ALCS employs proactive handover management. By maintaining an updated schedule of upcoming handover events, the algorithm can preemptively disable satellite links ahead of time, preventing packet loss and retransmissions during handovers. This strategy enhances overall transmission efficiency and reduces unnecessary resource consumption.    
\end{itemize}

Design details of the three components are elaborated in the following parts.

% An MPTCP sender stores packets both in its connection-level send buffer and in the subflow level send buffer (if the packet is assigned to that subflow). This means that if the number of packets in the connection level send buffer is larger than the aggregate number of packets in the subflow level send buffers, there are packets in the send buffer that need to be scheduled to the subflows.

\subsection{Latency Estimation for Satellite and Terrestrial Paths}
% Let us delve into the cases where $cwnd_f$ is not currently sufficient to transfer the data segment waiting to be sent.
% Despite the satellite subflow's advantage in terms of RTT, its CWND may sometimes be relatively smaller compared to the terrestrial subflow, given the limited bandwidth resource of the LEO satellite network.
% In situations where $cwnd_f$ is not sufficient to accommodate the data segment waiting to be sent, the ALCS we proposed endeavors to weigh the trade-off between latency and throughput when deciding which subflow to use for the pending data transmission. 

We assume that $k$ packet segments in the MPTCP connection level send buffer are waiting to be scheduled to the best available subflow. Similar to the default minRTT scheduler, if the fastest subflow \textemdash characterized by the minimal RTT \textemdash has available CWND space, ALCS would readily assign the packets to that subflow. However, in cases where the faster subflow $S_f$ lacks sufficient CWND space, ALCS would not allocate the data packets in the send buffer to the slower subflow $S_s$ immediately.

Instead, in cases where $cwnd_f$ is insufficient for the pending data, carefully balances the trade-off between latency and throughput before deciding on which subflow to send the packets.
Beyond just RTT and CWND, ALCS also considers the number of inflight packets and the queue length in the send buffer for each subflow. These additional factors allow ALCS to build a more comprehensive view of each subflow's state, leading to more informed decision-making. Once this analysis is completed, ALCS computes the end-to-end latency for transmitting the data segment over both subflows, denoted as $tl_f$ and $tl_s$ for $S_f$ and $S_s$, respectively. 

Given the assumption that there are $k$ data segments awaiting allocation, the calculation of $tl_f$ and $tl_s$ is given as
\begin{align}
    &tl_f=\frac{k+i_f+q_f}{cwnd_f}*(rtt_f+\Delta_f), \label{eq:ori-estimate-tlf} \\
    &tl_s=\frac{k+i_s}{cwnd_s}*(rtt_s+\Delta_s).\label{eq:ori-estimate-tls}
\end{align}
Here, $i_f$ and $i_q$ represent the number of inflight packets for subflows $S_f$ and $S_s$, respectively, and $q_f$ indicates the number of packets queued in the send buffer of $S_f$. The subflow expected to deliver the segment in the shortest total time is selected for transmission.

\subsection{Adaptive Estimated Latency Compensation}
% However, given the volatile characteristics of LEO satellite links, RTT-dependent estimations can occasionally be imprecise. This inaccuracy arises because RTT is derived from the difference between the time a data packet is transmitted and the time its corresponding ACK(acknowledgment) is received. Relying solely on historical knowledge to make strategies determining current or near-future actions may sometimes lead to less than suboptimal outcomes.
% The potential discrepancy between the estimated and actual RTT can impact the ALCS's ability to predict the optimal subflow for minimizing the end-to-end latency. The scheduler may inadvertently select a subflow that, while appearing to offer the fastest projected arrival time, may ultimately experience unexpected delays due to the volatile nature of the satellite link.

To address potential discrepancies between estimated and actual RTT, our scheduling approach integrates an adaptive latency compensation mechanism to refine latency estimates and mitigate the negative impact of RTT variability. To elaborate, we introduce a latency compensation factor, $\sigma$, which is dynamically adjusted based on the difference between the estimated transmission latency and the actual observed delay during recent transfer intervals. Initially, $\sigma_f$ and $\sigma_s$ are set to $1.0$ in ALCS. 

Within the ALCS framework, this adjustment process involves systematically assessing the variance between observed and predicted end-to-end transmission latencies at regular intervals. This is achieved by comparing the number of data packets successfully transmitted (denoted as $atp$ for ``actually transmitted packets'') with the expected number of dispatched packets (denoted as $etp$ for ``expected transmitted packets'') within a defined update interval $T_u$.
% Within the ALCS framework, there is a systematic and ongoing assessment of the variance between the actual observed and predicted end-to-end transmission latencies in a regular manner. This assessment is facilitated by closely tracking the discrepancy between the number of data packets that are successfully transmitted (termed as $atp$, for actually transmitted packets) and the number that was anticipated to be dispatched (referred to as $etp$, for expected transmitted packets), all within a defined interval $T_u$. 
If $atp > etp$, it indicates that the transmission latency has been overestimated, prompting the compensation factor $\sigma$ to be decreased by multiplying it with an attenuation factor, $\alpha$. Conversely, if $atp < etp$, $\sigma$ is increased by dividing it by $\alpha$. This attenuation mechanism tempers the adjustments to avoid overcorrection, ensuring that latency estimates remain precise without introducing new inaccuracies. Consequently, ALCS strikes a balance between improving latency prediction accuracy and maintaining network robustness under fluctuating conditions.

By employing this approach, Eq. (\ref{eq:ori-estimate-tlf}) and (\ref{eq:ori-estimate-tls}) are reformulated as
\begin{align}
    &tl_f=\frac{k+i_f+q_f}{cwnd_f}*(rtt_f+\Delta_f)*\sigma_f,\label{eq:estimate-tlf} \\
    &tl_s=\frac{k+i_s}{cwnd_s}*(rtt_s+\Delta_s)*\sigma_s.\label{eq:estimate-tls}
\end{align}
$\sigma_f$ and $\sigma_s$ are updated at each $T_u$ interval as
\begin{align}
    &\sigma_f \leftarrow \left\{
    \begin{array}{rcl}\label{eq:update-sigma-f}
    \sigma_f*\alpha  &     & {apt_f > etp_f,}\\
    \sigma_f/\alpha  &     & {apt_f < etp_f.}
    \end{array} \right. \\
    &\sigma_s \leftarrow \left\{
    \begin{array}{rcl}\label{eq:update-sigma-s}
    \sigma_s*\alpha  &     & {apt_s > etp_s,}\\
    \sigma_s/\alpha  &     & {apt_s < etp_s.}
    \end{array} \right.
\end{align}

\subsection{Proactive Handover Management}

Last but not least, to mitigate the handover-induced severe retransmission problem described in Section \ref{bg}, ALCS includes a proactive handover management mechanism based on the predictable trajectories of satellite motion.

Specifically, ALCS maintains a 24-hour schedule of satellite movements to predict handover times accurately. It strategically deactivates the satellite link one RTT before an inter-satellite handover is expected. This preemptive deactivation minimizes disruptions to ongoing data transmissions by ensuring that the satellite path is disabled just before the handover occurs. The one RTT buffer period allows sufficient time for any in-flight data packets to be successfully transmitted, avoiding packet loss during the handover process. 

By leveraging this advanced knowledge of handover timing, ALCS ensures continuous end-to-end connectivity, facilitating seamless handovers at the application layer. This proactive approach improves data transmission reliability and significantly enhances the overall user experience.

\input{algorithm}

Details of the scheduling procedures are outlined in the accompanying pseudo-code for the proposed ALCS algorithm.

\section{Experimental Setup}\label{testbed}

In this section, we simulate a simplified STIN testbed using Docker \cite{docker} and Python3. Our proposed ALCS approach is implemented within the MPTCP Linux Kernel \cite{mptcp-linux-kernel} by modifying the MPTCP scheduler module.

\subsection{Experimental Settings}

The topology of our simplified STIN system is illustrated in Fig. \ref{topology}.
The satellite network comprises multiple interconnected Satellite Nodes ($sn$s), which establish links with both the Source ($src$) and the Destination ($dst$) via ground stations. In the meanwhile, the terrestrial network is depicted by several Terrestrial Nodes ($tn$s), interconnected through ground-based infrastructure, without loss of generality. By utilizing multiple interfaces of both $sn$s and $tn$s, communication between $src$ and $dst$ can effectively employ both satellite and terrestrial networks simultaneously, optimizing data transmission across both paths.
% the long-distance communication between the $src$ and $dst$ can be facilitated through both satellite and terrestrial networks in tandem.

% our simulated STIN, which harnesses both satellite and terrestrial networks in tandem through the use of multiple interfaces. 
% The terrestrial network is simplified by several terrestrial network nodes ($tn$s) connected through the ground-based infrastructures without losing generality.
%This illustration showcases the key components and interactions within the integrated network architecture. On the upper part, the satellite network segment is depicted, comprising multiple interconnected satellite nodes ($sn$s) that can establish links with the source ($src$) device. On the lower part, the terrestrial network segment is shown, consisting of terrestrial network nodes ($tn$s) connected through the ground-based infrastructures. This integrated architecture allows the $src$ and destination ($dst$) devices to utilize multiple transmission paths simultaneously, leveraging both the satellite and terrestrial networks.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{throughput-sat0.01.png}
%     \caption{Throughput comparison of different schedulers with loss rate of satellite network is set to $0.01\%$.}
%     \label{fig:throughput-sat0.01}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{throughput-sat0.5-v2.png}
%     \caption{Throughput comparison of different schedulers with loss rate of satellite network is set to $0.5\%$.}
%     \label{fig:throughput-sat0.5}
% \end{figure}

The experimental setup is designed to emulate the operational characteristics of the STIN system. In our configuration, the terrestrial link is specified with a bandwidth of 100 Mbps, and an RTT around 108ms, calculated based on geographical distance. The satellite link, meanwhile, is set with a bandwidth of 50 Mbps, and its RTT varies between 52ms and 68ms due to satellite movement, reflecting the dynamic nature of satellite communication networks. Furthermore, the terrestrial network is assigned a loss rate of 0.01\%. In parallel, to mimic the inherent variability of satellite links, the satellite path is tested under two distinct conditions, with loss rates of 0.01\% and 0.5\%, respectively.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth]{STIN-topology.png}
    \caption{Topology of the simulated STIN.}
    \label{topology}
    \vspace{-10pt}
\end{figure}

\subsection{Experimental Testbed}
% We have established a Docker-based testbed that emulates the key characteristics of the STIN, including diverse network paths with varying latency and bandwidth profiles. Each Docker container serves as a satellite network node or a terrestrial network node in the simulated STIN. Each node is furnished with one or multiple network interface cards, which are interconnected via bridges. To simulate the movement of satellites, we leverage the disconnection and re-connection of these bridges to represent the handover of satellite connections. This process is controlled by a Python script that maintains a timetable derived from real-world satellite movement trajectories. With this timetable, the script can orchestrate the precise timing of the bridge disconnection and re-connection events, more accurately replicating the dynamic nature of satellite link availability and performance in a real STIN environment. By dynamically breaking and re-establishing the connections between the virtual bridges, our testbed can faithfully reproduce the impact of satellite mobility on the STIN topology. This approach allows us to create a controlled and reproducible environment for comparing the behavior of different multipath schedulers under various conditions.

We establish a Docker-based testbed to provide a highly flexible and configurable platform for evaluating the performance of multipath transmission schedulers in the context of STIN. By leveraging containerization, each network node is defined with its own set of network interfaces and interconnections, simulating the diverse paths and varying performance characteristics inherent to satellite and terrestrial network segments. This modular architecture allows for seamless reconfiguration and scaling, facilitating the exploration of a wide range of STIN scenarios.

To create a realistic, controlled, and compatible testbed that accurately simulates dynamic STIN conditions and evaluates the performance of various multipath schedulers, we employ the following core techniques:
\begin{itemize}
    \item \textbf{Two-Line Element (TLE) data for satellite orbits}. The simulation incorporates TLE data from Starlink satellites to ensure an accurate representation of satellite positions and movements. TLE data provides precise orbital information, allowing the testbed to realistically simulate the mobility of $sn$s.    
    \item \textbf{Geospatial coordinates for terrestrial network nodes}. The testbed uses the latitude and longitude coordinates of real-world cities to set the positions of $tn$s, enabling more accurate simulations of communication between ground stations and satellites, and terrestrial nodes. 
    \item \textbf{Accurate delay calculation for satellite and terrestrial links}. Delays for both satellite and terrestrial links are calculated using actual distances. Satellite link delays are derived from TLE data to measure distances between $sn$s and ground stations, while terrestrial delays are based on the geographical distance between $tn$s. This ensures precise latency modeling within the network simulation.
    % Delays for both satellite and terrestrial links are determined by calculating the actual distances, using TLE data for the $sn$s and geospatial coordinates for the $tn$s. Satellite link delays are calculated using the distances between $sn$s and between $sn$s and ground stations, while terrestrial link delays depend on the distances between $tn$s. This allows for accurate representation of latency within the simulated network.  
    \item \textbf{Traffic control for network parameter management}. Traffic control for network parameter management. The Linux Traffic Control (TC) utility is used to manage network parameters, such as latency, bandwidth, and packet loss, for both satellite and terrestrial links. TC allows precise control over link characteristics, ensuring realistic simulation of network conditions.  
    % The Linux Traffic Control (TC) utility is a powerful command-line tool that allows for precise management and manipulation of network traffic within the system. We employ TC to configure link characteristics such as latency, bandwidth, and packet loss for both satellite and terrestrial connections.  
    \item \textbf{Script-driven simulation of satellite movement and dynamic network conditions}. A script-driven approach is employed to simulate satellite handovers by dynamically establishing and disconnecting network bridges between Docker containers. This technique accurately mirrors satellite trajectories and handover events as satellites move in and out of coverage areas, enabling a realistic assessment of how handovers affect network topology and path availability. Additionally, a Python script recalculates delays for both satellite and terrestrial links in real time, with updated values applied using the TC utility. This ensures that network conditions remain responsive to the continuous changes induced by satellite movement.    
    % The testbed uses a script-driven approach to manage the dynamic creation and disconnection of network bridges between Docker containers, simulating satellite handovers. It utilizes actual satellite trajectories to precisely simulate handover events as satellites enter and exit coverage areas. This approach effectively replicates the effects of handovers on network topology and path availability, offering a realistic test environment for assessing the robustness and adaptability of multipath schedulers. Additionally, as satellites move, the Python script recalculates delays for both satellite and terrestrial links in real time. These updated delays are then applied using the TC utility, ensuring that network conditions in the simulation remain responsive to satellite movement.    
    \item \textbf{MPTCP Linux Kernel v0.96 for multipath communication}. The MPTCP Linux Kernel~\cite{mptcp-linux} version 0.96 underpins the evaluation of multipath schedulers. This version supports the core functionality and APIs required to enable multipath communication. Its compatibility with Linux Kernel Long-Term Support (LTS) release v5.4.230 ensures a stable and widely adopted foundation for the testbed. This environment allows for the reliable and robust evaluation of multipath data transmission.
\end{itemize}

By applying these methodologies, the testbed offers a controlled, reproducible platform for systematically comparing scheduling algorithms across diverse STIN scenarios.



% The script-driven approach to simulating satellite mobility is a particularly noteworthy aspect of this testbed. By maintaining a timetable of satellite movement based on real-world trajectories, the testbed can accurately reproduce the handover events that occur as satellites move in and out of coverage. The dynamic disconnection and re-connection of virtual bridges within the Docker containers faithfully replicate the impact of these handovers on the network topology and path availability. This level of fidelity is crucial for evaluating the robustness and adaptability of multipath schedulers, as they must be able to seamlessly handle the unpredictable changes in network conditions introduced by satellite mobility. The controlled and reproducible nature of this testbed setup enables systematic comparison of different scheduling algorithms and their performance under various STIN scenarios.

% To closely approximate reality, the simulation of satellite positions and orbits is based on the Two-Line Element (TLE) data of the Starlink satellites. This allows for a more accurate representation of the dynamic positioning of the $sn$s within the network. Additionally, the latitude and longitude coordinates of several actual cities are used to specify the locations of the $tns$s. Using these geospatial data, the delays for both the satellite links and the terrestrial links can be precisely calculated. The satellite link delays are determined based on both the distances between the Satellite Nodes ($sn$s) and the distances between $sn$s and the ground stations, while the terrestrial link delays are calculated based on the distances between the Terrestrial network Nodes ($tn$s) themselves.

% The calculated satellite and terrestrial link delays are implemented using the Traffic Control (TC) utility in Linux. TC is a powerful command-line tool that allows for precise management and manipulation of network traffic within the system. In addition, TC is employed to set the bandwidth and loss rates for the satellite and terrestrial links. The delay calculation and implementation are also written in the aforementioned Python script, which also controls the satellite movement and handovers. Each time the satellite moves, the corresponding delays would be re-calculated and re-implemented, ensuring that the network conditions remain accurately simulated in response to the satellite's movement.

% The MPTCP Linux Kernel\cite{mptcp-linux} version 0.96 serves as the foundation for our evaluation of MPTCP schedulers, as it provides the core functionality and APIs required to enable multipath communication or data transmission. The MPTCP v0.96 release is designed to be compatible with the Linux Kernel Long-Term Support (LTS) release v5.4.230. This compatibility ensures that our evaluation environment is based on a stable and widely used Linux kernel, allowing us to leverage the robust set of features and capabilities provided by the LTS release.

\begin{figure*}[t!]
    \centering
    \vspace{-10pt}
    \begin{minipage}[b]{0.32\textwidth}
        \captionsetup{width=0.9\linewidth} 
        \centering
        \includegraphics[width=0.98\linewidth]{40M-0.01-performance.png}\label{fig:throughput-sat0.01-50-40M}\subcaption*{(a)} \\
        \includegraphics[width=0.98\linewidth]{40M-0.5-performance.png}\label{fig:throughput-sat0.5-50-40M}\subcaption*{(b)}
        \caption{
        % The average transfer completion time and throughput of ALCS compared to minRTT, RR, ECF, and BLEST when transferring a 40M file. (a)The loss rate of the satellite network is set to 0.01\%. (b)The loss rate of the satellite network is set to 0.5\%.
        Comparison of average transfer completion time and throughput for all algorithms when transferring a 40 MB file at different satellite network loss rates: (a) 0.01\%, (b) 0.5\%.}
        \label{fig:throughput-40M}
    \end{minipage}
    \begin{minipage}[b]{0.32\textwidth}
        \captionsetup{width=0.9\linewidth} 
        \centering
        \includegraphics[width=0.98\linewidth]{100M-0.01-performance.png}\label{fig:throughput-sat0.01-50-100M}\subcaption*{(a)} \\
        \includegraphics[width=0.98\linewidth]{100M-0.5-performance.png}\label{fig:throughput-sat0.5-50-100M}\subcaption*{(b)}
        \caption{Comparison of average transfer completion time and throughput for all algorithms when transferring a 100 MB file at different satellite network loss rates: (a) 0.01\%, (b) 0.5\%.
        }
        \label{fig:throughput-100M}
    \end{minipage}
    \begin{minipage}[b]{0.322\textwidth}
        \captionsetup{width=0.9\linewidth} 
        \centering
        \includegraphics[width=0.98\linewidth]{150M-0.01-performance.png}\label{fig:throughput-sat0.01-50-150M}\subcaption*{(a)} \\
        \includegraphics[width=0.98\linewidth]{150M-0.5-performance.png}\label{fig:throughput-sat0.5-50-150M}\subcaption*{(b)}
        \caption{Comparison of average transfer completion time and throughput for all algorithms when transferring a 150 MB file at different satellite network loss rates: (a) 0.01\%, (b) 0.5\%.}
        \label{fig:throughput-150M}
    \end{minipage}
    \vspace{-10pt}
\end{figure*}

\section{Evaluation Results}\label{results}

In this section, we conduct a comprehensive evaluation of the ALCS scheduler within the enhanced simulation environment outlined above. The performance of ALCS is compared against several alternative multipath scheduling approaches, as outlined below:
\begin{itemize}
    \item \textbf{minRTT}~\cite{mptcp-linux-kernel}: This scheduler prioritizes the subflow with the lowest observed RTT for data transmission. While it reduces latency, it may neglect higher-bandwidth paths that could offer superior performance.
    \item \textbf{RR}~\cite{mptcp-linux-kernel}: The RR scheduler distributes traffic evenly across all active subflows, regardless of the current network conditions. Though this ensures a balanced use of resources, it can lead to inefficient network utilization.     
    \item \textbf{ECF}~\cite{ecf}: The ECF scheduler dynamically estimates the completion time for each subflow, prioritizing the subflow expected to complete data transfers fastest by accounting for factors beyond just RTT and CWND.
    \item \textbf{BLEST}~\cite{blest}: The BLEST scheduler estimates the blocking time for each subflow using various network performance metrics. It selects the subflow that promises the highest throughput potential, rather than favoring the path solely based on lower latency.
\end{itemize}

Our evaluation focuses on the following key performance metrics:
\begin{itemize}
    \item \textbf{Transmission Completion Latency}: It measures the time taken for files of a fixed size to travel from $src$ to $dst$ within the simulated STIN. It reflects ALCS's ability to minimize transmission delays, which is crucial for low-latency applications.
    \item \textbf{Overall Throughput}: We evaluate the data transfer rates achieved by each scheduler. This ensures that the latency optimizations provided by ALCS do not compromise throughput, as maintaining high throughput is equally important for efficient data delivery in STIN.
    \item \textbf{Retransmission Rate}: This metric examines the effectiveness of handover management by comparing the retransmission rates of different MPTCP schedulers during handover events, providing insight into their ability to maintain reliable data transmission.
\end{itemize}
    % To assess the effectiveness of the handover management mechanism, we compare the retransmission rates of these MPTCP schedulers in the scenario where handover events occur during the data transmission process.  

% Additionally, other factors such as the fraction of data transferred via satellite paths and the impact of the number of subflows are discussed as well

Furthermore, we also examine the proportion of data transmitted over satellite paths and analyze the influence of varying the number of subflows on overall performance.

\subsection{Transfer time and network throughput of the schedulers}

We first assess the schedulers by comparing their average throughput and transmission completion time from $src$ to $dst$ within our simulated STIN testbed. These comparisons are visually represented in Fig. \ref{fig:throughput-40M}, \ref{fig:throughput-100M}, \ref{fig:throughput-150M}.  A more detailed breakdown of ALCS's performance relative to other schedulers across various scenarios is provided in Table \ref{tab:overall-performance}.

Notably, to comprehensively account for the impact of satellite motion, we accelerate the satellite movement during the experiments. Each of the three sets of experiments is conducted at different times, ensuring that the transmission process experiences diverse changes in STIN conditions. However, within each set, two sub-tests---one with a packet loss rate of 0.01\% and the other with 0.5\%---are carried out simultaneously, allowing for a direct comparison of scheduler performance under varying packet loss conditions.

\begin{table*}[t!]
  \centering
  \caption{Overall Performance of ALCS compared to minRTT, RR, ECF, and BLEST in different scenarios.}
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
          &       & \multicolumn{2}{c|}{loss rate of satellite network: 0.01\%} & \multicolumn{2}{c}{loss rate of satellite network: 0.5\%} \\
\cmidrule{2-6}          & MPTCP scheduler & \multicolumn{1}{l|}{completion time (s)} & \multicolumn{1}{l|}{average throughput(MB/s)} & \multicolumn{1}{l|}{completion time (s)} & \multicolumn{1}{l}{average throughput(MB/s)} \\
    \midrule
    \multicolumn{1}{r|}{\multirow{5}[2]{*}{file size: 40M}} & minRTT & 11.183 & 4.05 & 26.885 & 1.72 \\
          & RR & 13.045 & 3.58 & 27.533 & 1.65 \\
          & ECF   & 10.722 & 4.80 & 22.741 & 1.78 \\
          & BLEST & 9.103 & 5.59 & 21.482 & 2.12 \\
          & ALCS  & 6.257 & 7.93 & 18.719 & 2.47 \\
    \midrule
    \multicolumn{1}{r|}{\multirow{5}[2]{*}{file size: 100M}} & minRTT & 44.647 & 2.53 & 48.828 & 2.06 \\
           & RR    & 28.048 & 4.05 & 57.537 & 1.99 \\
          & ECF   & 22.169 & 5.06 & 56.401 & 1.99 \\
          & BLEST & 19.293 & 5.88 & 48.162 & 2.40 \\
          & ALCS  & 16.473 & 7.01 & 42.201 & 2.75 \\
    \midrule
    % \multicolumn{1}{r|}{\multirow{5}[2]{*}{file size: 150M}} & minRTT & 59.151 & 2.83 & 44.675 & 3.79 \\
    %       & RR & 41.102 & 4.07 & 44.022 & 3.79 \\
    %       & ECF   & 43.981 & 3.88 & 43.178 & 4.15 \\
    %       & BLEST & 41.239 & 4.07 & 35.112 & 4.77 \\
    %       & ALCS  & 31.302 & 5.38 & 30.403 & 5.56 \\
    \multicolumn{1}{r|}{\multirow{5}[2]{*}{file size: 150M}} & minRTT & 59.151 & 2.83 & 50.975 & 3.27 \\
          & RR & 41.102 & 4.07 & 51.816 & 3.27 \\
          & ECF   & 43.981 & 3.88 & 48.159 & 3.53 \\
          & BLEST & 41.239 & 4.07 & 42.424 & 3.97 \\
          & ALCS  & 31.302 & 5.38 & 38.286 & 4.39 \\
    \bottomrule
    \end{tabular}%
  \label{tab:overall-performance}%
\end{table*}%

Fig. \ref{fig:throughput-40M} presents a comparison of the average throughput and transfer completion time for a 40MB file transmission using ALCS and four other MPTCP schedulers, under satellite network loss rates of 0.01\% and 0.5\%. It is evident that the ALCS scheduler consistently achieves shorter completion times and higher throughput across both loss scenarios, outperforming the alternative scheduling approaches. This trend persists in the transmission of larger files, as shown in Fig. \ref{fig:throughput-100M} and Fig. \ref{fig:throughput-150M}, for 100MB and 150MB files, respectively.

As expected, an increase in the satellite network's loss rate leads to a reduction in average throughput and longer transfer times for all schedulers across the three file sizes. The higher loss rate reflects increased link instability, prompting a heavier reliance on the terrestrial path, which has a higher RTT than the satellite link. This shift contributes to the observed decline in throughput. Despite this, ALCS consistently outperforms its counterparts, maintaining higher throughput and demonstrating superior resilience to packet loss. This highlights ALCS's effectiveness in managing the dynamic network conditions typical of STIN, ensuring both robust and efficient data transmission.

% As expected, our observations indicate a decline in average throughput and an increase in transfer time as the satellite network's loss rate increases across all three file transfer scenarios. This can be attributed to the fact that higher loss rates suggest greater satellite link dynamics, compelling a greater reliance on the terrestrial path, which has a higher RTT compared to the satellite path. As a result, the increase in loss rate affects the overall network throughput negatively. 
% Nevertheless, in each scenario, our proposed ALCS approach demonstrates superior performance over other MPTCP schedulers. ALCS maintains higher overall network throughput even in conditions of packet loss, underscoring its robustness and efficiency in addressing the challenges posed by variable network conditions, particularly in the STIN environment.

As the file size increases from 40M to 150M, all schedulers exhibit a predictable rise in completion time and a corresponding decline in average throughput. However, the performance gap between ALCS and the other schedulers becomes more pronounced with larger file sizes. The greater the file size, the longer the transfer duration, reflecting the growing complexities and dynamics in the transmission process. Under such circumstances, traditional MPTCP scheduling algorithms tend to suffer from performance degradation. For instance, in the 150MB file transfer scenario, both ECF and BLEST demonstrate performance comparable to RR and minRTT. Notably, in the case of a 0.01\% satellite link loss rate, ECF requires even more time than RR, indicating suboptimal performance in this specific situation.

In contrast, ALCS consistently outperforms the other schedulers, demonstrating a clear advantage across all file sizes and loss rates. This superior performance suggests that ALCS is not only more scalable but also more capable of handling larger data transfers within STIN environments. Its robustness in managing varying data loads highlights its effectiveness in adapting to different network conditions and maintaining efficient data transmission.
% In contrast, ALCS consistently outperforms the other schedulers, demonstrating a clear advantage across all file sizes and loss rates. This superior performance of ALCS suggests greater scalability and more effective handling of larger data transfers within the STIN or satellite network environments, highlighting its robustness in managing varying data load conditions.

To summarize, our proposed ALCS consistently achieves higher average throughput and shorter transfer completion time compared to the other MPTCP schedulers, across all three file sizes and both loss rate conditions. For smaller files, such as 40MB, and with a lower loss rate of 0.01\%, ALCS delivers a significant performance boost, with 44.0\% and 31.4\% enhancements over minRTT and BLEST, respectively. Remarkably, even under more challenging conditions, including a higher loss rate of 0.5\% and larger file sizes of 150MB, ALCS continues to demonstrate a commendable performance increase, providing a 24.8\% improvement over minRTT and a 9.8\% advantage over BLEST. This consistent superior performance across varying conditions underscores the robustness and efficiency of the ALCS algorithm.

\subsection{Retransmission rate of the schedulers}

\begin{figure}[t!]
    \centering
\includegraphics[width=0.7\linewidth]{marked-retrans-rate.png}
    \caption{The comparison of retransmission rate with different schedulers.}
    \label{fig:retrans_rate}
    \vspace{-10pt}
\end{figure}

Furthermore, ALCS stands out by achieving the lowest overall retransmission rate and the fewest handover-induced retransmission rate compared to other schedulers, as illustrated in Fig. \ref{fig:retrans_rate}. Impressively, ALCS eliminates packet retransmissions caused by satellite handovers entirely. 

This impressive result is due to the proactive handover management mechanism integrated into ALCS. The algorithm preemptively deactivates the satellite path one RTT before a handover occurs and keeps it inactive until the handover process is complete. This strategy effectively minimizes the disruption caused by satellite handovers, reducing the need for retransmissions and enhancing the reliability of end-to-end communications.

In the STIN context, where retransmissions are predominantly triggered by satellite handovers, ALCS's approach addresses this issue directly, ensuring more stable and efficient data transmission.

% This is because the majority of retransmissions in the STIN context stem from satellite handovers, especially when handovers occur during the transmission process, as previously outlined in Section \ref{bg}.
% The significant reduction in retransmission rate is attributed to the proactive handover management mechanism embedded within the ALCS. This mechanism preemptively deactivates the satellite path one RTT ahead of an impending handover and sustains this inactive state until the handover process is fully completed. 
% By doing so, ALCS effectively mitigates the disruptive effects of satellite handovers on network traffic, thereby diminishing the need for retransmissions and bolstering the reliability of end-to-end communications.



\subsection{Fraction of data transferred over the satellite path}

\begin{figure}[t!]
\centering
\vspace{-12pt}
\subfloat[The loss rate of satellite network is set to 0.01\%.]{
    \includegraphics[width=0.7\linewidth]{marked-frac-over-sat-0.01.png}\label{fig:frac-over-sat-0.01}}\\
\subfloat[The loss rate of satellite network is set to 0.5\%.]{
    \includegraphics[width=0.7\linewidth]{marked-frac-over-sat-0.5.png}\label{fig:frac-over-sat-0.5}}
\caption{Fraction of Data Allocated to the Satellite Path based on Different Satellite Network's Loss Rates.}
\label{fig:frac-over-sat}
\vspace{-10pt}
\end{figure}

Fig. \ref{fig:frac-over-sat} displays the proportion of traffic allocated to the satellite path, which has a lower RTT, under varying satellite network loss rates of 0.01\% and 0.5\%. The results clearly demonstrate that the ALCS algorithm is more aggressive in exploiting the satellite path in comparison to other schedulers. This is particularly evident when the satellite link's condition is favorable. ALCS effectively leverages the satellite path's advantages to enhance data transmission efficiency when it outperforms the terrestrial path.


In contrast, in scenarios where the satellite path's loss rate significantly exceeds that of the terrestrial path, traditional schedulers like minRTT and RR  fail to adjust their allocation strategies effectively in response to the prevailing network conditions. On the other hand, ECF, BLEST, and ALCS adapt the proportion of traffic sent over the satellite path to account for the higher loss rate, thereby optimizing the overall performance by leveraging the strengths of each available network path. 

Notably, BLEST shows a tendency to favor the terrestrial path slightly more than the ECF scheduler in both the file-1 and file-2 transfer scenarios. Conversely, ALCS does not exhibit a fixed preference for either path. It demonstrates flexibility in its path selection, utilizing the satellite path the least during the file-1 transfer but not showing the same bias during the file-2 transfer. 
This adaptability indicates that ALCS's decision-making is influenced by the specific conditions and requirements of each transfer scenario, rather than adhering to a uniform strategy. This flexibility is a key feature of ALCS, allowing it to maximize overall efficiency under varying network conditions. 

\subsection{Performance analysis with multiple subflows}

\begin{figure}[t!]
\centering
\vspace{-10pt}
%\includegraphics[width=3in]{fig5}
\subfloat[Transfer completion time.]{
    \includegraphics[width=0.7\linewidth]{marked-multi-sf-time.png}\label{fig:multi-sf-time}}\\
\subfloat[Average throughput.]{
    \includegraphics[width=0.7\linewidth]{marked-multi-sf-throughput.png}\label{fig:multi-sf-throughput}}\\
\caption{Performance comparison of various schedulers under different numbers of subflows.}
\label{fig:performance-multiple-subflows}
\vspace{-10pt}
\end{figure}

We proceed to examine the impact of varying the number of subflows, as depicted in Fig. \ref{fig:performance-multiple-subflows}. This analysis explores how the number of subflows influences the overall performance and behavior of the MPTCP schedulers. The performance evaluation is conducted during the transfer of a 150MB file within the STIN environment, where the satellite network loss rate is set to 0.5\% while the terrestrial network loss rate is fixed at 0.01\%.

Fig. \ref{fig:multi-sf-time} compares transfer completion time across different schedulers, and Fig. \ref{fig:multi-sf-throughput} highlights their performance in terms of average throughput. As the number of subflows increases from 2 (1 satellite and 1 terrestrial path) to 4 (2 satellite and 2 terrestrial paths), there is a notable improvement in the overall performance of all MPTCP schedulers. With more subflows, the schedulers have access to a broader selection of network paths, allowing more efficient distribution of data load and better aggregation of bandwidth across the available subflows. For instance, if one of the satellite paths experiences a connection disruption, the scheduler can seamlessly switch to an alternative satellite path, maintaining end-to-end connectivity and minimizing communication interruptions. Moreover, the presence of additional subflows facilitates more effective load balancing, allowing data to be allocated dynamically across paths based on real-time network conditions.

However, further increasing the number of subflows from 4 to 6 results in a degradation of system performance. This decline can be attributed to the increased complexity of scheduling, load balancing, and congestion control across multiple paths. With more available active subflowsk, optimizing their usage becomes more challenging, potentially leading to suboptimal utilization of network resources. Notably, the issue of out-of-order packet delivery worsens when 6 subflows are active, suggesting that beyond a certain point, adding more subflows introduces more complexity than benefit, ultimately reducing overall system efficiency.

Despite these challenges, the proposed ALCS consistently outperforms other schedulers in all tested scenarios, excelling in both transfer completion time and average throughput. This highlights ALCS’s superior adaptability and efficiency, even in the presence of increasing subflow complexity.


% \begin{figure}[htbp]
% \centering
% %\includegraphics[width=3in]{fig5}
% \subfloat[minRTT]{
% 		\includegraphics[width=0.8\linewidth]{minrtt-cwnd-v1.png}}\label{fig:minrtt-cwnd}\\
% \subfloat[RR]{
% 		\includegraphics[width=0.8\linewidth]{rr-cwnd.png}}\label{fig:rr-cwnd}\\
% \subfloat[ECF]{
% 		\includegraphics[width=0.8\linewidth]{ecf-cwnd.png}}\label{fig:ecf-cwnd}\\
% \subfloat[BLEST]{
% 		\includegraphics[width=0.8\linewidth]{blest-cwnd-v1.png}}\label{fig:blest-cwnd}\\
% \subfloat[ALCS]{
% 		\includegraphics[width=0.8\linewidth]{alcs-cwnd.png}}\label{fig:alcs-cwnd}
% \caption{CWND trace of different schedulers over time.}
% \label{fig:cwnd-behavior}
% \end{figure}

% \begin{figure*}[t!]
%     \centering
%     \subfloat[minRTT]{
%         \includegraphics[width=0.325\textwidth]{minrtt-cwnd-v1.png}}\hfill
%     \subfloat[RR]{
%         \includegraphics[width=0.325\textwidth]{rr-cwnd.png}}\hfill
%     \subfloat[ECF]{
%         \includegraphics[width=0.325\textwidth]{ecf-cwnd.png}}
    
%     \vspace{-0.5em}

%     \hfill
%     \subfloat[BLEST]{
%         \includegraphics[width=0.33\textwidth]{blest-cwnd-v2.png}}\hfill
%     \subfloat[ALCS]{
%         \includegraphics[width=0.33\textwidth]{alcs-cwnd.png}}
%     \hspace{2cm}
%     \caption{CWND trace of different schedulers over time.}
%     \label{fig:cwnd-behavior}
% \end{figure*}

\section{Discussion and Future Work}\label{discussion}

\textbf{Applicability to diverse networks.}
% ALCS demonstrates exceptional adaptability to various traffic patterns, making it highly effective not only within the specialized STIN framework for file transmission and data segment scheduling but also across a wide range of network environments. Its utility extends to common terrestrial networks, such as Wi-Fi and LTE, where it can enhance performance under diverse conditions. Given its proven ability to handle different transfer sizes efficiently, ALCS offers significant performance improvements for numerous network-based applications and services. For instance, it can enhance the user experience in audio and video streaming by reducing latency and buffering, and it ensures smoother and more responsive web browsing for online applications. Moreover, ALCS excels in managing large file transfers, making it particularly valuable for use cases such as software updates, cloud storage synchronization, and media distribution. This versatility positions ALCS as a robust solution capable of meeting a broad spectrum of network-based demands.
ALCS demonstrates exceptional adaptability to various traffic patterns, making it effective not only within the STIN framework for file transmission and data segment scheduling but also across diverse network environments. Its utility extends to common terrestrial networks like Wi-Fi and LTE, enhancing performance under varying conditions. With its capability to efficiently handle different transfer sizes, ALCS significantly improves performance for numerous applications. For instance, it reduces latency and buffering in audio and video streaming, ensuring smoother web browsing experiences. Additionally, ALCS excels in managing large file transfers, making it valuable for software updates, cloud storage synchronization, and media distribution. This versatility positions ALCS as a robust solution for a wide range of network-based demands.

% \textbf{Applicability to diverse networks.} ALCS showcases robust adaptability to a range of traffic patterns. Although it is particularly well-suited for efficient file transmission and data segment scheduling within the STIN framework, its utility is not confined to this specialized environment. ALCS can be effectively applied across a variety of network conditions, including the ubiquitous terrestrial Wi-Fi and LTE connections. In the meanwhile, given its demonstrated adaptability to diverse transfer sizes, ALCS can boost the performance of numerous network-based applications and services. It can significantly improve the user experience in audio and video streaming, and allows for a more responsive and fluid browsing experience for web-based applications. Additionally, due to its proficiency in managing large file transfers, ALCS is beneficial for various use cases such as software updates, cloud storage synchronization, and media distribution. This versatility makes ALCS a robust solution for a diverse range of network-based needs.


\textbf{Integration with MPTCP.} The core logic of ALCS has been implemented as a new scheduling module in the MPTCP Linux Kernel as mentioned in Section \ref{testbed}. This implementation ensures the seamless integration of ALCS within the MPTCP framework, leveraging the existing functionality and infrastructure of the MPTCP protocol. Moreover, the MPTCP framework provides a scalable and extensible foundation, allowing the ALCS scheduling module to be efficiently deployed and scaled to accommodate varying network loads and workloads. This seamless integration enhances the robustness and flexibility of ALCS in real-world applications. 

\textbf{Limitation and Future Work.} The current ALCS design is primarily focused on optimizing transfer completion time, a critical factor that directly impacts user experience, particularly for latency-sensitive applications. While reducing transfer delays can significantly enhance user satisfaction, it is acknowledged that other performance metrics, such as fairness and energy efficiency, may also be essential in certain contexts. As such, future iterations of the ALCS scheduler would aim to balance and optimize these additional metrics, adopting a more holistic approach to improving user experience. This would involve not only optimizing speed but also ensuring the equitable distribution of network resources and minimizing energy consumption.

Building on existing efforts, exploring the interplay between congestion control and packet scheduling across multiple paths in the STIN environment holds significant promise. This investigation is a natural extension of ALCS's current design, which already considers key path characteristics such as RTT, CWND, and in-flight packets—critical factors in developing effective congestion control algorithms.
While we currently use established algorithms like Cubic, along with multipath-specific methods such as Balia \cite{balia} and Olia \cite{olia}, our findings indicate that these approaches yield suboptimal performance in STIN. 
% CWND often declines over time or remains confined to a low range, highlighting the inadequacy of existing congestion control algorithms in this context. 
Therefore, it is imperative to develop a new congestion control algorithm specifically tailored to the unique challenges of STIN. Such an algorithm, integrated with ALCS, would further enhance multipath transmission performance and resilience, ensuring robust, efficient data transfer even in highly dynamic network conditions.
% Currently, we utilize the widely deployed congestion control algorithm Cubic \cite{cubic}, as well as multipath-specific congestion control methods such as Balia\cite{balia} and Olia\cite{olia}, to model the window behavior of ALCS subflows.
% However, our observations show that these algorithms perform suboptimally in the STIN environment, with CWND either persistently declining over time or remaining confined to a low range, demonstrating poor performance of already-existed congestion control algorithms when deployed in STIN. 



\section{Related Work} \label{related-work}
% Numerous congestion control algorithms tailored for MPTCP, such as OLIA, BALIA, D-LIA, and so forth, have also been proposed to ensure fair bandwidth utilization compared to a single TCP connection within a shared communication environment.

\textbf{Multipath extensions over TCP.}
% MPTCP is a major extension of the traditional TCP protocol, designed to leverage multiple network paths between two end hosts for the transfer of a single data stream. It was formally standardized by the Internet Engineering Task Force in 2013~\cite{rfc8684}. Since then, MPTCP has been integrated into various operating systems, including Linux~\cite{mptcp-linux-kernel}, Apple iOS and macOS~\cite{ios-mptcp}, FreeBSD~\cite{freebsd-mptcp}, and Solaris~\cite{solaris-mptcp}. Over the years, MPTCP has also become a significant area of research, with ongoing efforts from the academic and engineering communities aimed at improving the protocol's performance and functionality. Key areas of focus include optimizing path management, enhancing data scheduling, and refining congestion control mechanisms.
MPTCP is a significant extension of traditional TCP, designed to leverage multiple network paths between two end hosts for transferring a single data stream. Standardized by the Internet Engineering Task Force in 2013~\cite{rfc8684}, MPTCP has been integrated into various operating systems, including Linux~\cite{mptcp-linux-kernel}, FreeBSD~\cite{freebsd-mptcp}, and Solaris~\cite{solaris-mptcp}. Over the years, it has become a prominent research area, with ongoing efforts from academia and industry to enhance its performance and functionality. Key focus areas include optimizing path management, improving data scheduling, and refining congestion control mechanisms.

% In general, the MPTCP study can be divided into three main sections, including path manager, data scheduler, and congestion controller. 

% \textbf{Path management in MPTCP.}
% The MPTCP path manager is responsible for detecting and establishing available end-to-end paths based on certain pre-defined criteria. For example, the Fullmesh path manager endeavors to create all possible subflows when establishing the MPTCP connection, while the Ndiffports path manager is designed to flexibly adapt to different network conditions by dynamically adjusting the number of established subflows according to the user requirements. 

% \textbf{Congestion control in MPTCP.}
% In shared communication environments, fairness in bandwidth utilization has been a key challenge. To address this issue, numerous congestion control algorithms tailored for MPTCP have been proposed, such as OLIA, BALIA, and D-LIA. By considering the dynamics of the available paths, these methods strive to achieve more equitable resource sharing among different subflows.

\textbf{Packet scheduling in MPTCP.} 
% As the focal point of this paper, packet scheduling is a critical component that directly influences the performance of any MPTCP transport system. 
Packet scheduling is a crucial element that significantly impacts the performance of MPTCP transport systems. In recent years, substantial research has been devoted to advancing packet scheduling algorithms for MPTCP. Kuhn et al. \cite{daps} propose a delay-aware packet scheduling algorithm to handle path heterogeneity in forward delay and CWND, ensuring in-order packet delivery. Similarly, Yang et al.~\cite{otia} introduce a scheduler that predicts the arrival time of each packet at the receiver and prioritizes subflows based on the shortest predicted arrival time. Other schedulers such as STMS~\cite{stms} and DEMS~\cite{dems} have also been developed to reduce out-of-order arrivals. STMS prioritizes the faster subflow for packet allocation and uses the slower subflow to transmit packets with larger sequence numbers. DEMS splits a data chunk across two subflows and strategically decouples the paths for chunk delivery efficiency.
% The ECF scheduler \cite{ecf} addresses performance degradation arising from path heterogeneity by minimizing the waiting time on the faster subflow. 
Similar to ECF, STTF, proposed by Hurtig et al. \cite{sttf}, aims to reduce the transmission time of each data segment by considering the current congestion state of each subflow, and dynamically adjusting to network conditions. Moreover, several loss-aware schedulers integrate loss rates into their decision-making process for selecting subflows and prioritizing paths with the lowest estimated delay for segment transmission~\cite{lamps, late}. Various machine learning-based approaches have also been applied to MPTCP packet scheduling~\cite{olaps, reles, peekaboo}. 
% Xing et al.~\cite{olaps} develop an online learning-based scheduler that optimizes packet scheduling by modeling it as a multi-armed bandit problem, generating adaptive policies to quickly respond to abrupt network changes. 
% Zhang et al.~\cite{reles} propose a reinforcement learning-based MPTCP scheduler entailing an asynchronous training algorithm, enabling parallel execution of packet scheduling, data collecting, and neural network training to optimize the scheduling strategy. 

\textbf{Multipath transmission within STIN.} The application of multipath transmission protocols such as MPTCP and multipath QUIC \cite{de2017multipath} (MPQUIC) in the context of STIN remains a relatively underexplored area compared to their extensive application in terrestrial networks. Xiao et al.~\cite{xiao2022efficient} introduce an MPTCP scheme based on an SDN architecture to enhance the throughput and efficiency in STIN, while Wang et al.~\cite{cdmr} propose a computing-dependent multipath routing paradigm to optimize task computing during end-to-end transmission. Yang et al. develop a mobility-aware MPQUIC framework, along with customized data scheduling~\cite{mams-quic} and congestion control algorithms~\cite{ma-quic}, specifically tailored to the unique end-to-end path conditions within STIN.
The limited research on multipath transmission in STIN highlights the need for further exploration and innovative solutions. 
% Critical areas such as multipath packet scheduling, path management, and congestion control remain underdeveloped, underscoring the potential for significant advancements in optimizing performance across these integrated networks.
% The relative scarcity of research on multipath transmission within STIN underscores the need for deeper investigation and innovative approaches, particularly concerning multipath packet scheduling, path management, congestion control, and other related aspects to optimize performance in these integrated networks.



\section{Conclusion} \label{conclusion}

In this work, we present an analytical framework for MPTCP-enabled STIN and demonstrate the performance degradation of several traditional existing MPTCP schedulers when deployed in STIN environments. To address the three key challenges posed by STIN—severe path heterogeneity, high volatility, and frequent handovers—we introduce a STIN-optimized multipath scheduling approach called ALCS. ALCS addresses path heterogeneity by integrating RTT, CWND, inflight packets, and queuing delay to estimate transmission delays across subflows. These estimates are further refined using latency compensation mechanisms to mitigate the unpredictable nature of satellite links. In addition, ALCS incorporates a proactive handover management strategy that leverages the predictability of satellite movement to effectively manage frequent handovers.
Through experiments conducted in our custom-built testbed, we evaluate ALCS against the minRTT, RR, ECF, and BLEST schedulers, focusing on metrics such as transfer completion time, average throughput, and retransmission rate under various network conditions. The results consistently demonstrate the superior performance of ALCS, delivering improvements ranging from 9.8\% to 44.0\% over the baseline algorithms across different scenarios.

==> problem-equation.tex <==
\begin{align*}
\text{Minimize } & D = \sum_{i=1}^{n} \sum_{j=1}^{P} D_{ij} = \sum_{i=1}^{n} \sum_{j=1}^{P} X_{ij} \cdot \left( RTT_{ij} + \frac{B_i}{CWND_{ij}} \right) \\
\text{Subject to } & \\
& \sum_{i=1}^{n} B_i = B, \quad \forall i  \\
& D_{ij} \geq 0, \quad \forall i, j \\
& \sum_{i=1}^{n} \sum_{j=1}^{P} B_i \cdot CWND_{ij} \geq B \\
& \sum_{j=1}^{P} X_{ij} = 1, \quad \forall i \\
& X_{ij} \in \{0, 1\}, \quad \forall i, j \\
\end{align*}

\begin{equation*}
\begin{aligned}
& \text{Minimize} && D = \sum_{n=1}^{N} \left( \sum_{j=1}^{S} X_{ij} \left( \frac{B_n}{C_{ij}} + \frac{B_n}{C_{gj}} \right) + (1 - X_{ij}) \frac{B_n}{C_{gi}} \right) \\
& \text{subject to} && \\
& && 0 \leq B_n \leq B, \quad \forall n \\
& && \sum_{n=1}^{N} B_n = B \\
& && \sum_{n=1}^{N} X_{ij} \cdot B_n \leq C_{ij}, \quad \forall j \\
& && \sum_{n=1}^{N} (1 - X_{ij}) \cdot B_n \leq C_{gi}, \quad \forall j \\
& && X_{ij} \in \{0, 1\}, \quad \forall i, j \\
\end{aligned}
\end{equation*}
